DNS-based Ingress Load Balancing: An Experimental Evaluation

Multihomed services can load-balance their incoming connection requests using DNS, resolving the name of the server with different addresses depending on the link load that corresponds to each address. Previous work has studied a number of problems with this approach, e.g., due to Time-to-Live duration violations and client proximity to local DNS servers. In this paper, we experimentally evaluate a DNS-based ingress traffic engineering system that we deployed at Georgia Tech. Our objective is to understand whether simple and robust load balancing algorithms can be accurate in practice, despite aforementioned problems with DNS-based load balancing methods. In particular, we examine the impact of various system parameters and of the main workload characteristics. We show that a window-based measurement scheme can be fairly accurate in practice, as long as its window duration has been appropriately configured.

==> Makefile <==
REPORT=main
LATEX=latex
BIBTEX=bibtex --min-crossrefs=1000
REF1=ref

TEX = $(wildcard *.tex)
CLS = $(wildcard *.cls)
SRCS = $(TEX)
REFS=$(REF1).bib

all: pdf
#.tex.dvi:
#       $(LATEX) $*.tex

#$(REPORT).dvi: figures $(SRCS) $(CLS) paper.bib
$(REPORT).dvi: $(SRCS) $(CLS) $(REF1).bib
	$(LATEX) $(REPORT)
	$(BIBTEX) $(REPORT)
	perl -pi -e "s/%\s+//" $(REPORT).bbl
	$(LATEX) $(REPORT)
	$(LATEX) $(REPORT)

#$(REPORT).ps: $(REPORT).dvi figures
$(REPORT).ps: $(REPORT).dvi 
	dvips -Pcmz -t letter $(REPORT).dvi -o $(REPORT).ps
#	dvips -Ppdf -G0 -t letter $(REPORT).dvi -o $(REPORT).ps



#not relevant here
#figures:
#	cd figures; make


view: $(REPORT).dvi
	xdvi $(REPORT).dvi

print: $(REPORT).dvi
	dvips $(REPORT).dvi

pdf: $(REPORT).ps
	ps2pdf14 -dPDFSETTINGS=/prepress -dSubsetFonts=true -dEmbedAllFonts=true $< $(REPORT).pdf

printer: $(REPORT).ps
	lpr $(REPORT).ps

tidy:
	rm -f *.dvi *.aux *.log *.blg *.bbl

clean:
	rm -f *~ *.dvi *.aux *.log *.blg *.bbl $(REPORT).ps $(REPORT).pdf $(PROPOSAL).ps $(PROPOSAL).pdf $(FIRSTDRAFT).ps $(FIRSTDRAFT).pdf



